LithOS: An Operating System for Efficient Machine Learning on GPUs

The surging demand for GPUs in datacenters for machine learning (ML) has made efficient GPU utilization crucial. However, meeting the diverse needs of ML models while optimizing resource usage is challenging. To enable transparent, fine-grained GPU management that maximizes utilization and energy efficiency while maintaining strong isolation, an operating system (OS) approach is needed. This paper introduces LithOS, a first step toward a GPU OS. LithOS includes the following new abstractions and mechanisms for efficient GPU resource management: (i) a novel TPC Scheduler that supports spatial scheduling at the granularity of individual TPCs, unlocking efficient TPC stealing between workloads; (ii) transparent kernel atomization to reduce head-of-line blocking and enable dynamic resource reallocation mid-execution; (iii) a lightweight hardware right-sizing mechanism that determines the minimal TPC resources needed per atom; and (iv) a transparent power management mechanism that reduces power consumption based on in-flight work behavior. We implement LithOS in Rust and evaluate its performance across extensive ML environments, comparing it to state-of-the-art solutions from NVIDIA and prior research. For inference stacking, LithOS reduces tail latencies by 13x compared to MPS; compared to the best SotA, it reduces tail latencies by 3x while improving aggregate throughput by 1.6x. In hybrid inference-training stacking, LithOS reduces tail latencies by 4.7x compared to MPS; compared to the best SotA, it reduces tail latencies 1.18x while improving aggregate throughput by 1.35x. Finally, for a modest performance hit under 4%, LithOS's right-sizing provides a quarter of GPU capacity savings on average, while for a 7% hit, its power management yields a quarter of a GPU's energy savings. Overall, LithOS increases GPU efficiency, establishing a foundation for future OS research on GPUs.

==> Discussion.tex <==

\section{Discussion and Future Work}

\mypar{Other GPU Resources.}  This paper focuses on scheduling compute. Techniques for managing other resources are orthogonal and can be integrated into \arch{}. Prior work has focused on GPU memory~\cite{10.1145/3620666.3651353, tgs, nvshare, bakita-ssd, rt-swap}, memory bandwidth~\cite{fgpu, missle}, PCIe ~\cite{missle, rgem}, SSDs~\cite{bam, bakita-ssd}, and networking~\cite{298709}. We believe that \arch{} is a first step towards an operating system that can virtualize additional resources.

\mypar{On-device Scheduling.} While \arch{} currently runs on CPU cores, an interesting future direction is to offload parts of its functionality onto the GPU itself. This shift could be particularly beneficial as CPU-GPU integration becomes tighter, as seen in NVIDIA’s superchip architecture~\cite{superchip}. However, this design space presents trade-offs—balancing the efficiency of running the control plane on lightweight GPU cores against the flexibility and performance of traditional CPU cores. We leave this exploration for future work. 

\mypar{Software / Hardware Co-design.} \arch{} focuses on existing hardware architectures and provides mechanisms and abstractions that can benefit current and future GPU architectures. However, there are several features of \arch{} that could be performed directly on the GPU without any CPU intervention. While this is not feasible with existing hardware, we believe that \arch{} will open up a new direction for operating systems research, which, coupled with hardware extensions, will lead to additional efficiency gains.



